Structural properties of the first-order transduction quasiorder

Logical transductions provide a very useful tool to encode classes of structures inside other classes of structures. In this paper we study first-order (FO) transductions and the quasiorder they induce on infinite classes of finite graphs. Surprisingly, this quasiorder is very complex, though shaped by the locality properties of first-order logic. This contrasts with the conjectured simplicity of the monadic second order (MSO) transduction quasiorder. We first establish a local normal form for FO transductions, which is of independent interest. Then we prove that the quotient partial order is a bounded distributive join-semilattice, and that the subposet of \emph{additive} classes is also a bounded distributive join-semilattice. The FO transduction quasiorder has a great expressive power, and many well studied class properties can be defined using it. We apply these structural properties to prove, among other results, that FO transductions of the class of paths are exactly perturbations of classes with bounded bandwidth, that the local variants of monadic stability and monadic dependence are equivalent to their (standard) non-local versions, and that the classes with pathwidth at most $k$, for $k\geq 1$ form a strict hierarchy in the FO transduction quasiorder.

==> locality.tex <==
\subsection{Locality of stability and dependence}
%\label{sec:monlocal}


\begin{lemma}
If a class $\Cc$ of graphs is independent, then there is a strongly local
formula that is independent. 
\end{lemma}
\begin{proof}
Assume $\phi(\bar x,y)$ is independent over $\Cc$. 
		We rewrite $\phi(\overline x,y)$ in Gaifman normal 
		form as a Boolean combination of basic local sentences and $r$-local formulas. By an easy argument, we reduce to the case where the formula is $r$-local. 
		By a standard Ramsey argument we can select a subsequence such that the every subset of size $p$ of the $\overline a_i$ is order-indiscernible for formulas with quantifier rank $r$. Let $b$ be a vertex adjacent to all $\overline a_i$ with even $i$ and to none with odd $i$. We rewrite $\phi(\overline x,y)$ as a Boolean combination of strongly local formulas. We can then extract a subsequence such that for some of these formula $\psi$, $\psi(\overline a_i,b)$ alternates between true (for even indices) and false (for even ones). Using order-indiscernibility, we find all the needed $b_J$ (by reducing the global size from $p$ to $p/3$).
		Thus we found a strongly local independent formula.
		\end{proof}
	

\begin{corollary}
A class of graphs is dependent if and only if it is locally dependent.
\end{corollary}

\begin{lemma}
If a class of graphs is unstable, then there is a strongly local
formula that is unstable. 
\end{lemma}
\begin{proof}
By applying Gaifman's Theorem, we rewrite the formula as a Boolean combination of sentences and $r$-local formulas. By an easy argument, we reduce to the case where the formula is $r$-local.

It will be convenient to introduce, 
for a graph $F$ with vertex set $[n]$ and $r\in\mathbb N$, the formula
\[
	\zeta_{r,F}(x_1,\dots,x_n):=\biggl(\bigwedge_{\{i,j\}\in E(F)}{\rm dist}(x_i,x_j)\leq r\biggr)\wedge\biggl(\bigwedge_{\{i,j\}\notin E(F)}{\rm dist}(x_i,x_j)>r\biggr).
\]

	
		By a standard Ramsey argument, if $n>f(p)$ we can find a graph $F$ and $1\leq i_1<\dots<i_p\leq n$ such that 
	$G\models\zeta_{2r,F}(\overline a_{i_j},\overline a_{i_k},\overline a_{i_\ell})$ for every $1\leq j<k<\ell\leq p$. (It follows that $F$ has a symmetric structure.) 
	We define $\overline b_j=\overline a_{i_j}$. We consider the connected components of $F$.
	Let $m=|\overline a_i|$. If $\alpha$ and $\beta+m$ are adjacent in $F$ (for some $1\leq \alpha,\beta\leq m$ then $\alpha+m$ is adjacent to $\beta+2m$ and $\alpha$ is adjacent to $\beta+2m$ hence $\alpha,\alpha+m,\alpha+2m,\beta,\beta+m$, and $\beta+2m$ belong to the same connected component of $F$. The partition of $[3m]$ into connected components consists of parts of the form $A\cup(A+m)\cup (A+2m)$ and of triples of parts of the form $A$, $(A+m)$ and $(A+2m)$ (for some $A\subseteq [m]$). It follows that $\phi(\overline x,\overline y)$ is equivalent, on the tuples $\overline b_i$ to a Boolean combination of strongly local formulas involving the same indices for $\overline x$ and $\overline y$ for parts of the first kind, or involving only some indices of $\overline x$ or of $\overline y$ in the second case. By Ramsey argument, we can assume that the satisfaction of these formulas only depend on the order of the $\overline b_i$. At least one of these is thus antisymmetric. It follows that there exists a strongly local formula $\psi(\overline x',\overline y')$ with the order property (with $|\overline x'|\leq |\overline x|$ and $|\overline y'|\leq |\overline y|$).
\end{proof}

\begin{corollary}
A class of graphs is stable if and only if it is locally stable.
\end{corollary}

%\begin{example}
%	It is known that unit interval graphs have locally bounded rankwidth. Actually, it is easily checked that they have locally bounded linear rankwidth.
%\end{example}
%
%Consider a class $\mathscr C$ 

==> monadic.tex <==
\section{Stability, dependence, and their local variants}
\label{sec:monlocal}
The notions of stability and dependence are two of the most important notions
in classification theory~\cite{shelah1990classification}. The notions of \emph{monadic stability} and \emph{monadic dependence} were studied
by Baldwin and Shelah in~\cite{baldwin1985second} and naturally fit
into the framework of transductions. 
In this paper, we introduced some local versions and have shown (\cref{thm:local}) that 
a class of graphs is monadically stable (resp.\ monadically dependent) 
if and only if it is locally monadically stable (resp.\ locally monadically dependent). In fact, 
we will prove now that more generally, a class of graphs is stable (resp.\ dependent) 
if and only if it is locally stable (resp.\ locally dependent). The proof of this 
more general fact is based on a standard Ramsey argument, while the
monadic cases illustrate nicely the use of our transduction normal form. 

Before proceeding to the proof, we take time to recall basic definitions related to stability and dependence.
Note that the standard notions of stability and dependence concern first-order theories. However, the stability (resp. dependence) of a theory can be alternatively defined by some characteristic properties of its models, namely that every formula has bounded order property \cite{shelah1990classification} (resp. is dependent) on every model. This justifies the extension of the notion of stability and dependence to classes of graphs, with the property that a first-order theory (in the language of graphs) is stable (resp. dependent) if and only if the class of its models is stable (resp. dependent).
\subsection{Stability and monadic stability}
\begin{definition}
Let $\Cc$ be a class of $\Sigma$-expanded graphs. A formula 
$\phi(\bar x,\bar y)$ with $|\bar x|=|\bar y|=k$
has the \emph{$n$-order property} over $\Cc$ 
if there exists $G\in\Cc$ and $\bar a_1,\ldots, 
\bar a_n\in V(G)^k$ such that $G\models\phi(\bar a_i,\bar a_j)$ if and only
if $i<j$. The formula $\phi$ has the \emph{order property} if it has 
the $n$-order property for all $n\geq 1$. %A class $\Cc$ has the ($n$-)order
%property if there exists a $\Sigma$-formula which has the ($n$-)order property
%over $\Cc$. 
\end{definition}

Recall that the half-graph $H_n$ has vertices $a_1,\ldots, a_n, b_1,\ldots, b_n$ and 
edges $\{a_i,b_j\}$ for $i\leq j$. Observe that for a graph $G$ and a formula $\phi(\bar x,\bar y)$, 
if we have $\bar a_1,\ldots, \bar a_n\in V(G)^{|\bar x|}$ and 
$\bar b_1,\ldots, \bar b_n\in V(G)^{|\bar y|}$ such that 
$G\models\phi(\bar a_i,\bar b_j)\Leftrightarrow i\leq j$, then the formula
$\psi(\bar x_1\bar y_1,\bar x_2\bar y_2)\coloneqq \phi(\bar x_1,\bar y_2)
\wedge \neg\phi(\bar x_2,\bar y_2)$ has the $n$-order property as witnessed
by $\bar a_1\bar b_1, \ldots, \bar a_n\bar b_n$. 


\begin{definition}
A class $\Cc$ of $\Sigma$-expanded graphs is {\em stable} if 
no $\Sigma$-formula $\phi(\bar x,\bar y)$ with $|\bar x|=|\bar y|=k$ 
has the order property over $\Cc$. 
%there is an integer $n$ such that for every graph $G\in\Cc$ there exist no $2n$ tuples $\bar a_1,\dots,\bar a_n,\bar b_1,\dots,\bar b_n$ in $V(G)^k$ with the property that $G\models \phi(\bar a_i,\bar b_j)$ if and only if $i\leq j$.
\end{definition}

\begin{definition}
A class $\Cc$ of $\Sigma$-expanded graphs is {\em monadically stable} 
if every monadic expansion of $\Cc$ is stable.
\end{definition}

%In model theory we usually do not deal with classes of graphs (or structures), but 
%rather with theories. However, we can naturally associate with every first-order 
%theory $T$ the class~$\Cc_T$ of its (finite and infinite) models. Then the definition 
%of the $n$-order property, order property and stability naturally extends from 
%classes of graphs to theories, e.g., a theory $T$ is stable if $\Cc_T$ is stable. 
%%Hence, we say that a theory $T$ %has the ($n$-)order property or that $T$ 
%%is stable if $\Cc_T$ %has the ($n$-)order property or 
%%is stable. 
%By compactness, if $T$ is a theory, then if a formula $\phi$ has the order property, then there exist $(\bar a_i)_{i\in \N}$ in a model $G$ of $T$ such that $G\models \phi(\bar a_i,\bar a_j)$
%if and only if~$i<j$ (and this is the original definition from model theory). 
%However, this is not relevant for our work. 

%\begin{definition}
%A class $\Cc$ of $\Sigma$-colored graphs is {\em monadically stable} if 
%for every monadic expansion $\Sigma^+$ and for every $\Sigma^+$-formula $\phi(\bar x,\bar y)$ with $|\bar x|=|\bar y|=k$ there is an integer $n$ such that for every graph $G\in\Cc$ and every monadic expansion $G^+$ of $G$ there exist no $2n$ tuples $\bar a_1,\dots,\bar a_n,\bar b_1,\dots,\bar b_n$ in $V(G)^k$ with the property that $G^+\models \phi(\bar a_i,\bar b_j)$ if and only if $i\leq j$.
%\end{definition}
%In other words, a class $\Cc$ is monadically stable if every monadic expansion of $\Cc$ is stable.

The next theorem, though stated for a theory, easily extends to general classes of structures.
\begin{theorem}[\cite{baldwin1985second}]
\label{thm:ms}
If a theory $T$ is not monadically stable, then there is a first-order formula~$\psi(x,y)$ with only two free variables and with monadic parameters that has the order property (for an appropriate interpretation of the monadic parameters).
\end{theorem}

%The graph $H_n$ with vertices $a_1,\ldots, a_n, b_1,\ldots, b_n$ and 
%edges $\{a_i,b_j\}$ for $i\leq j$ is called a {\em half-graph} of length $n$ \cite{HG}. Observe that for a graph $G$ and a formula $\phi(\bar x,\bar y)$, 
%if we have $\bar a_1,\ldots, \bar a_n\in V(G)^{|\bar x|}$ and 
%$\bar b_1,\ldots, \bar b_n\in V(G)^{|\bar y|}$ such that 
%$G\models\phi(\bar a_i,\bar b_j)\Leftrightarrow i\leq j$, then the formula
%$\psi(\bar x_1\bar y_1,\bar x_2\bar y_2)\coloneqq \phi(\bar x_1,\bar y_2)
%\wedge \neg\phi(\bar x_2,\bar y_2)$ has the $n$-order property as witnessed
%by $\bar a_1\bar b_1, \ldots, \bar a_n\bar b_n$. For monadic stability the
%situation is even simpler. For a graph $G$ and a formula $\phi(x,y)$ with 
%two free variables, 
%if we have $a_1,\ldots, a_n\in V(G)$ and 
%$b_1,\ldots, b_n\in V(G)$ such that 
%$G\models\phi(a_i,b_j)\Leftrightarrow i\leq j$, we can mark the 
%$b_i$ with a monadic predicate $B$. Then $\psi(x,y)\coloneqq 
%\forall z (B(z)\rightarrow (\phi(z,y)\rightarrow \phi(z,x))$ has the $n$-order
%property as witnessed by $a_1,\ldots, a_n$. Hence, orders and half-graphs
%can be used interchangeably. 


For a graph $G$ and formula $\phi(x,y)$ with 
two free variables, 
if we have $a_1,\ldots, a_n\in V(G)$ and 
$b_1,\ldots, b_n\in V(G)$ such that 
$G\models\phi(a_i,b_j)\Leftrightarrow i\leq j$, we can mark the 
$a_i$'s with a predicate $A$ and the $b_j$'s with a monadic predicate $B$. Then 
the interpretation $\mathsf I=(A(x)\vee B(x), A(x)\wedge B(y)\wedge \phi(x,y)\vee A(y)\wedge B(x)\wedge \phi(y,x))$ maps the marked graph to the half-graph $H_n$. We deduce the following corollary of \cref{thm:ms}.


\begin{corollary}
\label{cor:MS}
	For a class of finite graphs $\Cc$, the following are equivalent:
	\begin{enumerate}
		\item $\Cc$ is monadically stable,
		\item there is no transduction from $\Cc$ onto the class $\mathscr H$ of half-graphs.
	\end{enumerate}
\end{corollary}


%\begin{remark}
%	One could wonder how \cref{thm:ms}, which concerns theories, implies \cref{cor:MS}, which concerns (possibly non-definable) classes of finite graphs. In particular, the use of a monadic expansion makes it difficult to apply arguments based on ultra-products and {\L}o\'s's theorem.
%The proof of \cref{thm:ms} is based on Ramsey arguments, like the extraction of order-indiscernible sequences. 
%%Based on a comprehensive exposition of \cref{thm:ms} by Anderson \cite{anderson1990tree}, a finitary graph version of \cref{thm:ms} is presented for completeness in \cref{sec:appMS}. A similar treatment can be performed on  \cref{thm:md}, but we decided not include it as it proceeds in a very similar way as the rewriting of the proof of \cref{thm:ms} presented in the appendix.
%\end{remark}


%\section{Monadic dependence}
\subsection{Dependence and monadic dependence}
\begin{definition}
Let $\Cc$ be a class of $\Sigma$-expanded graphs. A
formula $\phi(\bar x,\bar y)$
has the \mbox{\emph{$n$-independence property}} over $\Cc$ 
if there exists $G\in\Cc$ and $\bar a_1,\ldots, 
\bar a_n\in V(G)^{|\bar x|}$ and $\bar b_J\in V(G)^{|\bar y|}$ for 
$J\subseteq [n]$ such that $G\models\phi(\bar a_i,\bar b_J)$ if and only
if $i\in J$. The formula $\phi$ has the \emph{independence property} if it has 
the $n$-independence property for all $n\in\N$. %A class $\Cc$ has the ($n$-)order
%property if there exists a $\Sigma$-formula which has the ($n$-)order property
%over $\Cc$. 
\end{definition}

\begin{definition}
A class $\Cc$ of $\Sigma$-expanded graphs is {\em dependent} if 
no formula $\phi(\bar x,\bar y)$
has the independence property over $\Cc$. 
%there is an integer $n$ such that for every graph $G\in\Cc$ there exist no $2n$ tuples $\bar a_1,\dots,\bar a_n,\bar b_1,\dots,\bar b_n$ in $V(G)^k$ with the property that $G\models \phi(\bar a_i,\bar b_j)$ if and only if $i\leq j$.
\end{definition}

\begin{definition}
A class $\Cc$ of $\Sigma$-expanded graphs is {\em monadically dependent} if 
if every monadic expansion of $\Cc$ is dependent.
\end{definition}

While it is well known that for dependence it is 
sufficient to consider formulas $\phi(\bar x;\bar y)$ with $|\bar y|=1$, it is not possible in general to reduce further to  
formulas $\phi(x,y)$ with only two free variables. However, as mentioned before, this is possible when we consider monadic dependence. Again, the next theorem, though stated for a theory, easily extends to general classes of structures.

%\begin{lemma}[Lemma 2.5; Lecture Notes on NIP Theories]
%The formula $\phi(\bar x;\bar y)$ has IP if and only if there is an indiscernible sequence $(\bar a_i: i<\omega)$ and a tuple $\bar b$ such that
%\[
%\models \phi(\bar a_i;\bar b)\quad\iff\quad i\text{ is even}.
%\]
%\end{lemma}
%
%\begin{lemma}[Proposition 2.6; Lecture Notes on NIP Theories]
%	The formula $\phi(\bar x;\bar y)$ is NIP if and only if any indiscernible sequence $(\bar a_i: i\in \mathcal I)$ and tuple $\bar b$, there is some end segment $\mathcal I_0$ and some $\eta\in\{0,1\}$ such that $\phi(\bar a_i;\bar b)^\eta$ holds for any $i\in\mathcal I_0$.
%\end{lemma}
%
%It is well known that it is sufficient to test all formulas $\phi(\bar x;\bar y)$ with $|\bar x|=1$.
%
\begin{theorem}[\cite{baldwin1985second}]
\label{thm:md}
	If a theory $T$ is monadically independent, then there is a first-order formula $\psi(x,y)$ with monadic parameters that has the independence property (for an appropriate interpretation of the monadic parameters).
\end{theorem}
%\begin{proof}
%	If $\Cc$ is not dependent then there is a formula $\phi(x, \bar y)$ with the property that for each integer $n$ there is some $G\in\Cc$ and some $\{\bar a_i\mid 1\leq i\leq n\}$ and some $\{b_I\mid I\subseteq [n]\}$ such that $i\in I$ if and only if $G\models \phi(b_I,\bar a_i)$. We prove by induction on $k=|\bar x|$ that this implies the existence of a first order formula $\psi(x,y)$ with additional unary predicates, such that\dots.
%	
%	If $k=1$, we have nothing to prove.
%	Let $P$ be the subset of all even integers in $[n]$, and let $b=b_P$. Then $\phi(b,\bar a_{2i})\wedge\neg \phi(b,\bar a_{2i+1})$.
%\end{proof}

\begin{corollary}
	\label{cor:MNIP}
	Let $\Cc$ be a class of graphs. Then the following are equivalent:
	\begin{enumerate}
		\item $\Cc$ is monadically dependent,
		\item there is no transduction from $\Cc$ onto the class $\Gg$ of all finite graphs.
	\end{enumerate}
\end{corollary}


==> more.tex <==
\section{Graph version of Theorem~\ref{thm:ms}}
\label{sec:appMS}
The  proof of the finitary graph version of \cref{thm:ms} presented here is based on Anderson's comprehensive exposition~\cite{anderson1990tree}.

\begin{definition}
	Two $k$-tuples $\bar{s}$ and $\bar{t}$ of integers have the same {\em order type} if, for every $1\leq i<j\leq k$ we have that $(s_j-s_i)$ is positive (resp.\ zero, resp.\ negative) if and only if $(t_j-t_i)$ is positive (resp.\ zero, resp.\ negative).
\end{definition}

\begin{definition}
	Let $k$ be an integer and let $\Delta$ be a finite set
	of formulas $\phi(\bar{x}_1,\dots,\bar{x}_p)$ with $|\bar{x}_1|=\dots=|\bar{x}_p|=k$.
	%
	A sequence $(\bar{a}_i)_{i\in I}$  of $k$-tuples of vertices of a graph $G$ is {\em  $\Delta$-order-indiscernible} if for every 
	$\phi(\bar{x}_1,\dots,\bar{x}_p)\in\Delta$
	and every two $p$-tuples $(i_1,\dots,i_p),(j_1,\dots,j_p)$ of elements of $J$ with same order type we have
\[
 G\models \phi(\bar{a}_{i_1},\dots,\bar{a}_{i_p})\longleftrightarrow\phi(\bar{a}_{j_1},\dots\bar{a}_{j_p}).
\]
\end{definition}


\begin{notation}
	For a formula $\phi(\bar{x}_1,\dots,\bar{x}_p)$ with $|\bar{x}_1|=\dots=|\bar{x}_p|=k$ and a permutation $\sigma$ of $[p]$ we denote by $\phi_\sigma$ the formula 
$
\phi_\sigma(\bar{x}_1,\dots,\bar{x}_p)=\phi(\bar{x}_{\sigma(1)},\dots,\bar{x}_{\sigma(p)})$.
\end{notation}


Let $R_{k,p}(n)$ denote the minimum order of a set $K$, such that for every coloration of the $i$-tuples 
 of $K$ in $k$ colors (for each $i\leq p$) there exists in $K$ a subset $K'$ of size $n$, such that for each $i\leq p$ all the $i$-tuples in $K'$ have the same color.

\begin{lemma}
\label{lem:Ramsey}
	Let $k,p\geq 2$ be integers and let $\Delta$ be a finite set
	of formulas $\phi(\bar{x}_1,\dots,\bar{x}_q)$ with $q\leq p$ and $|\bar{x}_1|=\dots=|\bar{x}_q|=k$.
For every integer $n\geq 3$ there is an integer $N\leq R_{2^{p!|\Delta|+k^2},p}(n)$ with the following property:

For every sequence $(\bar{a}_i)_{i\in I}$ of $k$-tuples of vertices, with $I\subseteq\mathbb N$ and $|I|\geq N$.  there exists $J\subseteq I$ with $|J|=n$ such that
\begin{enumerate}
	\item the sequence $(\bar{a}_i)_{i\in J}$ is $\Delta$-order-indiscernible;
	\item either there is an integer $s$ such that the $s$-th coordinate of all the  $\bar{a}_i$'s  are the same, or all the $\bar{a}_i$'s are disjoint (as sets).
\end{enumerate}	
\end{lemma}
\begin{proof}
	Let $\bar{\Delta}$ be the set of formulas
\[\bar{\Delta}=\Delta\cup\{\varphi_\sigma\mid \varphi(\bar{z})\in\Delta, \sigma\in\mathfrak{S}_{|\bar{z}|/k}\}\cup\{\eta_{i,j}\mid i,j\in [k]\},\]
where $\eta_{i,j}(\bar{x},\bar{y}):=(x_i=y_j)$ (where $x_i$ is the $i$th coordinate of $\bar{x}$ and $y_j$ is the $j$th coordinate of $\bar{y}$).
Assume $I\subseteq\mathbb N$ has cardinality at least $R_{2^{|\bar{\Delta}|,p}}(n)\leq R_{2^{p!|\Delta|+k^2},p}(n)$.

	We color the $q$-subsets of  $I$ as follows: for $1\leq i_1<i_2<\dots<i_q\leq n$, the color of the subset $\{i_1,\dots,i_q\}$ by the vector of the truth value of $\phi(\bar{a}_{i_1},\dots,\bar{a}_{i_q})$ for $\phi(\bar{x}_1,\dots,\bar{x}_q)\in\Delta$.
		
	According to Ramsey theorem, $I$ contains a subset $J$ of order $n$ such that for each $i\leq p$ the $i$-subsets of $J$ have all the same color.
	
	It is immediate that $J$ satisfies condition (1).
	 
	 
	Assume that for some $s,t\in[k]$ we have $G\models\eta_{s,t}(\bar{a}_i,\bar{a}_j)$ for every $i<j$ in $J$. Then, as $n\geq 3$, there exists $i<j<k$ in $J$ such that $G\models\eta_{s,t}(\bar{a}_i,\bar{a}_j)\wedge \eta_{s,t}(\bar{a}_i,\bar{a}_k)$
	hence the $t$-th coordinate of $\bar{a}_j$ and $\bar{a}_k$ are the same, hence (considering $\eta_{t,t}$)  the $t$-th coordinate of all the $\bar{a}_i$'s are the same.
	Otherwise, all the $\bar{a}_i$'s are disjoint as sets. Thus (2) holds.
\end{proof}

We shall need the following technical lemma:

\begin{lemma}
\label{lem:PsiChi}
	Let $k,r$ be integers, let $I\subseteq\mathbb N$ with $|I|=n$, let $\Delta$ be the set of all formulas 
	$\varphi(\bar{x}_1,\dots,\bar{x_q})$ with $1\leq q\leq 3$ and  $|\bar{x}_1|=\dots=|\bar{x}_p|=k$ and $\mathrm{qrank}(\varphi)\leq r$, 
	and let $(\bar{a}_i)_{i\in I}$ be
		a $\Delta$-indiscernible sequence of disjoint $k$-tuples of $G$.
	For $i\in I$ denote by $\bar{b}_i$ and $c_i$ the initial $(k-1)$-tuple and the last element of $\bar{a}_i$ (so that $\bar{a}_i=\bar{b}_ic_i$).


Assume $J\subseteq I$ is such that $\min I$ and $\max I$ are not in $J$, and between any two elements of $J$ there is an element of $I$. 	Let $\bar{J}=\{i\in I\mid \min J\leq i\leq \max J\}$.


Then either there exists a monadic lift of $G$ with $k+1$ unary predicates and a formula $\varphi(\bar{x}',\bar{y'})$ with $|\bar{x'}|=|\bar{y'}|<k$ such that $\varphi$ linearly orders a set of tuples indexed by $J$, 
or for every formulas $\Psi(\bar{x})$ ($|\bar{x}|=k$) and $\chi(y,z)$ with at most two parameters $\bar{a}_\alpha$ and $\bar{a}_\beta$ (with  $\alpha$ and $\beta$ in $I\setminus\bar{J}$)
and  quantifier rank at most $r-2$, and for every elements  $s\neq t$ in $J$ we have
\begin{enumerate}[(i)]
	\item\label{enum:psi1} $G\models \Psi(\bar{b}_sc_t)\longleftrightarrow\Psi(\bar{b}_tc_s)$;
	\item\label{enum:psi2} $G\models \Psi(\bar{b}_sc_s)\longleftrightarrow\Psi(\bar{b}_sc_t)$;
	\item\label{enum:chi} $G\models\chi(c_s,c_t)\longleftrightarrow \chi(c_t,c_s)$.
\end{enumerate}
\end{lemma}
\begin{proof}
	Assume \eqref{enum:psi1} fails for some admissible $\Psi$. Without loss of generality $G\models \Psi(\bar{b}_sc_t)\wedge\neg\Psi(\bar{b}_tc_s)$ (otherwise consider $\neg\Psi$).  We consider the case where $s<t$ (the case where $t<s$ is proved similarly). 
	As $(\bar{a}_i)_{i\in I}$ is $\Delta$-indiscernible,
 for every $i<j$ in $\bar{J}$  we have $G\models \Psi(\bar{b}_ic_j)\wedge \neg\Psi(\bar{b}_jc_i)$.
	For every $u<v$ in $J$ there exists $w\in\bar{J}$ such that
	$u<w<v$. Then $G\models \Psi(\bar{b}_uc_w)$ and $G\models \neg\Psi(\bar{b}_vc_w)$. Conversely, if $G\models \Psi(\bar{b}_uc_w)$ and $G\models \neg\Psi(\bar{b}_vc_w)$ for some $w\in \bar{J}$ then 
	$u<w$ and $w<v$. Let $Q=\{c_i\mid i\in \bar{J}\}$ and let
\[
\varphi(\bar{x}',\bar{y}'):=(\exists z\in Q)\ (\Psi(\bar{x}'z)\wedge\Psi(\bar{y}'z)),
\]	
where $|\bar{x}'|=|\bar{y}'|=k-1$.
Then $\varphi$ linearly orders $\{\bar{b}_i\mid i\in J\}$ (which has size $|J|$ as the $\bar{a}_i$'s are disjoint). (The parameters in $\Psi$ are eliminated by using $2k$ new unary predicates.)

Otherwise, assume that for some admissible $\Psi$ 
\eqref{enum:psi1} holds but \eqref{enum:psi2} fails.
Without loss of generality $G\models \Psi(\bar{b}_sc_t)\wedge\neg\Psi(\bar{b}_sc_s)$. We consider the case where $s<t$ (the case where $t<s$ is proved similarly).
By $\Delta$-indiscernibility, for every $i<j$ in $\bar{J}$  we have $G\models \Psi(\bar{b}_ic_j)\wedge \neg\Psi(\bar{b}_ic_i)$.
In particular, if $i<s$ we have $G\models \Psi(\bar{b}_ic_s)$. If $j>s$, as $G\models \Psi(\bar{b}_sc_j)$ we get from \eqref{enum:psi1} that $G\models\Psi(\bar{b}_jc_s)$.
It follows that $c_s$ is the unique solution of $\neg\Psi(\bar{b}_sz)\wedge Q(z)$. Hence 
$\{\bar{b}_i\mid i\in J\}$ is linearly ordered by 
\[
\varphi(\bar{x}',\bar{y}'):=(\exists w,z\in Q)\ (\neg\Psi(\bar{x}'w)\wedge\neg\Psi(\bar{y}'z)\wedge\phi(\bar{x}'w,\bar{y}'z))
\]
(Again, the parameters in $\Psi$ are eliminated by using $k$ new unary predicates.)

Assume \eqref{enum:chi} fails for some admissible $\chi$. Without loss of generality $G\models \chi(c_s,c_t)\wedge\neg\chi(c_t,c_s)$. Then $\chi(x,y)$ linearly orders the set $Q$ (which has size $|\bar{J}|\geq |J|$ as the $\bar{a}_i$'s are disjoint).
\end{proof}
\begin{theorem}
		Let $\phi(\bar{x},\bar{y})$ be a formula such that $|\bar{x}|=|\bar{y}|=k$. Then for every integer $n$ there exists $N=N(n,k)$ with the following property:
		
		For every graph $G$, if $\phi$ linearly orders a set of $N(n,k)$ $k$-tuples in $G$ then there exists a formula $\varphi(x,y)$  with at most $2k$ new unary predicates and quantifier rank at most $\mathrm{qrank}(\phi)+2(k-1)$,
	such that $\varphi$ linearly orders a subset of $n$ individuals of a monadic expansion of $G$.
\end{theorem}
\begin{proof}
	Assume for contradiction that the theorem does not hold, and assume $k$ is minimal in the sense that there exists no $N'=N'(n,k)$ such that for every graph $G$, if $\phi$ linearly orders a set of $N'(n,k)$ $k$-tuples in $G$ then there exists a formula $\varphi(\bar{x}',\bar{y}')$  with at most $2$ new unary predicates, quantifier rank at most $\mathrm{qrank}(\phi)+2$, and $|\bar{x}'|=|\bar{y}'|\leq k-1$, 
	such that $\varphi$ linearly orders a subset of $n$ individuals of a lift of $G$.
	
		Let $(\bar{a}_i)_{i\in I_0}$ be a sequence of $k$-tuples of $G$ linearly ordered by $\phi$, where $$|I_0|\geq R_{2^{2|\Delta|+k^2}}(2(N'(n,k-1)+2)(N'(n,k-1)+1)+2).$$ According to Lemma~\ref{lem:Ramsey} there exists a subset $I\subseteq I_0$ of size at least $6N'(n,k-1)+2$ such that the sequence $(\bar{a}_i)_{i\in I}$ is $\Delta$-order indiscernible (where $\Delta$ is the set of all formulas $\varphi(\bar{x},\bar{y})$ with $|\bar{x}|=|\bar{y}|=k$ and $\mathrm{qrank}(\varphi)\leq \mathrm{qrank}(\phi)+2$) and either there is an integer $s$ such that the $s$-th coordinate of all the  $\bar{a}_i$'s  are the same, or  all the $\bar{a}_i$'s are disjoint.
		
		If the $s$-th coordinate of all the  $\bar{a}_i$'s  are the same we can mark this element using a unary predicate and linearly order the $(k-1)$-tuples obtained by removing the $s$-th coordinate from the $\bar{a}_i$'s, contradicting the minimality assumption on $k$.
		
		Let $J_0$ be the subset of $I$ obtained by selecting one vertex over two, starting from the second vertex in $I$. Note that $|J_0|=(N'(n,k-1)+2)(N'(n,k-1)+1)$, and let $J_1$ be the subset of $J_0$ containing one element over $N'(n,k-1)+1$, starting from the $N'(n,k-1)+1$-th.
		Then, according to Lemma~\ref{lem:PsiChi} and the minimality assumption on $k$, the properties \eqref{enum:psi1},\eqref{enum:psi2}, and \eqref{enum:chi} stated in Lemma~\ref{lem:PsiChi} hold for every
		$J\subseteq J_0$ of order at least $N'(n,k-1)$, and any  admissible $\Psi$ and $\chi$. 
		
		
		Now we claim that if $u,s,t,v\in J_1$ are such that  $u<s<t<v$ or $v<s<t<u$ we have 
		$G\models \phi(\bar{b}_sc_u,\bar{b}_tc_v)$. This will be proved using a chain of similar statements (with same conclusion but different assumptions on the order type of $(s,t,u,v)$):
		\begin{itemize}
			\item If $s=u<t=v$ then $G\models \phi(\bar{b}_sc_u,\bar{b}_tc_v)$ as $\bar{b}_sc_u=\bar{a}_u$ and $\bar{b}_tc_v=\bar{b}_t$;
			\item If $u<s<t=v$ then by  Property~\eqref{enum:psi2} Lemma~\ref{lem:PsiChi} for 
			$J=\{i\in J_0\mid i<t\}$ and  
			$\Psi(\bar{x}):=\phi(\bar{x},\bar{b}_tc_v)$ (parameter $\bar{a}_t$) we have $G\models \Psi(\bar{b}_sc_s)\longleftrightarrow \Psi(\bar{b}_sc_u)$, i.e. $G\models\phi(\bar{b}_sc_s,\bar{b}_tc_v)\longleftrightarrow \phi(\bar{b}_sc_u,\bar{b}_tc_v)$. 
			From the previous item we have $G\models \phi(\bar{b}_sc_s,\bar{b}_tc_v)$ thus $G\models \phi(\bar{b}_sc_u,\bar{b}_tc_v)$.
			\item[$\circledast$] If $u<s<t<v$  then by Property~\eqref{enum:psi2} Lemma~\ref{lem:PsiChi} for 
			$J=\{i\in J_0\mid i>s\}$ and $\Psi(\bar{x}):=\phi(\bar{b}_sc_u,\bar{x})$ (parameters $\bar{a}_u$ and $\bar{a}_s$) we have $G\models \Psi(\bar{b}_tc_t)\longleftrightarrow \Psi(\bar{b}_tc_v)$, i.e. $G\models\phi(\bar{b}_sc_u,\bar{b}_tc_t)\longleftrightarrow \phi(\bar{b}_sc_u,\bar{b}_tc_v)$. From the previous item we have $G\models \phi(\bar{b}_sc_u,\bar{b}_tc_t)$ thus $G\models \phi(\bar{b}_sc_u,\bar{b}_tc_v)$.
		\item If $s<u<t<v$ then by Property~\eqref{enum:psi1} Lemma~\ref{lem:PsiChi} for 
			$J=\{i\in J_0\mid i<t\}$ and $\Psi(\bar{x}):=\phi(\bar{x},\bar{b}_tc_v)$ (parameters $\bar{a}_t$ and $\bar{a}_v$) we have $G\models \Psi(\bar{b}_uc_s)\longleftrightarrow \Psi(\bar{b}_sc_u)$, i.e. $G\models\phi(\bar{b}_uc_s,\bar{b}_tc_v)\longleftrightarrow \phi(\bar{b}_sc_u,\bar{b}_tc_v)$. From the previous item we have $G\models \phi(\bar{b}_uc_s,\bar{b}_tc_v)$ thus $G\models \phi(\bar{b}_sc_u,\bar{b}_tc_v)$.
		\item If $s<u<v<t$ then by 
			Property~\eqref{enum:psi1} Lemma~\ref{lem:PsiChi} for 
			$J=\{i\in J_0\mid i>u\}$ and $\Psi(\bar{x}):=\phi(\bar{b}_sc_u,\bar{x})$ (parameters $\bar{a}_s$ and $\bar{a}_u$) we have $G\models \Psi(\bar{b}_vc_t)\longleftrightarrow \Psi(\bar{b}_tc_v)$, i.e. $G\models\phi(\bar{b}_sc_u,\bar{b}_vc_t)\longleftrightarrow \phi(\bar{b}_sc_u,\bar{b}_tc_v)$. From the previous item we have $G\models \phi(\bar{b}_sc_u,\bar{b}_vc_t)$ thus $G\models \phi(\bar{b}_sc_u,\bar{b}_tc_v)$.
			\item If $s<v<u<t$ then by 
			Property~\eqref{enum:chi} Lemma~\ref{lem:PsiChi} for 
			$J=\{i\in J_0\mid s<i<t\}$ and
			$\chi(x,y):=\phi(\bar{b}_sx,\bar{b}_ty)$ (parameters $\bar{a}_s$ and $\bar{a}_t$) we have $G\models \chi(c_v,c_u)\longleftrightarrow \chi(c_u,c_v)$, i.e. $G\models\phi(\bar{b}_sc_v,\bar{b}_tc_u)\longleftrightarrow \phi(\bar{b}_sc_u,\bar{b}_tc_v)$. From the previous item we have $G\models \phi(\bar{b}_sc_v,\bar{b}_tc_u)$ thus $G\models \phi(\bar{b}_sc_u,\bar{b}_tc_v)$.
		\item If $v<s<u<t$ then by 
			Property~\eqref{enum:psi1} Lemma~\ref{lem:PsiChi} for 
			$J=\{i\in J_0\mid i<u\}$ and $\Psi(\bar{x}):=\phi(\bar{x}'c_u,\bar{b}_tx'')$ (parameters $\bar{a}_u$ and $\bar{a}_t$, $\bar{x}=\bar{x}'x''$) we have $G\models \Psi(\bar{b}_vc_s)\longleftrightarrow \Psi(\bar{b}_sc_v)$, i.e. $G\models\phi(\bar{b}_vc_u,\bar{b}_tc_s)\longleftrightarrow \phi(\bar{b}_sc_u,\bar{b}_tc_v)$. From the previous item we have $G\models \phi(\bar{b}_vc_u,\bar{b}_tc_s)$ thus $G\models \phi(\bar{b}_sc_u,\bar{b}_tc_v)$.
		\item[$\circledast$] If $v<s<t<u$ then by Property~\eqref{enum:psi1} Lemma~\ref{lem:PsiChi} for 
			$J=\{i\in J_0\mid i>s\}$ and $\Psi(\bar{x}):=\phi(\bar{b}_sx'',\bar{x}'c_v)$ (parameters $\bar{a}_s$ and $\bar{a}_v$, $\bar{x}=\bar{x}'x''$) we have $G\models \Psi(\bar{b}_uc_t)\longleftrightarrow \Psi(\bar{b}_tc_u)$, i.e. $G\models\phi(\bar{b}_sc_t,\bar{b}_uc_v)\longleftrightarrow \phi(\bar{b}_sc_u,\bar{b}_tc_v)$. From the previous item we have $G\models \phi(\bar{b}_sc_t,\bar{b}_uc_v)$ thus $G\models \phi(\bar{b}_sc_u,\bar{b}_tc_v)$.
		\end{itemize}
	
Then, reversing the ordering and replacing $\phi(\bar{x},\bar{y})$ by $\neg\phi(\bar{y},\bar{x})\wedge(\bar{x}\neq\bar{y})$ we obtain
\[
(v<t<s<u\text{ or }u<t<s<v)\rightarrow G\models\neg\phi(\bar{b}_tc_v,\bar{b}_sc_u).
\]
Altogether if we fix $u=\min J_1$ and $v=\max J_1$ then the formula $\phi(\bar{x}'c_u,\bar{y}'c_v)$ linearly orders the set $\{\bar{b}_i\mid u<i<v\}$.

This final contradiction completes the proof of the theorem.

\end{proof}
